Fast Robust Subspace Tracking via PCA in Sparse Data-Dependent Noise

This work studies the robust subspace tracking (ST) problem. Robust ST can be simply understood as a (slow) time-varying subspace extension of robust PCA. It assumes that the true data lies in a low-dimensional subspace that is either fixed or changes slowly with time. The goal is to track the changing subspaces over time in the presence of additive sparse outliers and to do this quickly (with a short delay). We introduce a "fast" mini-batch robust ST solution that is provably correct under mild assumptions. Here "fast" means two things: (i) the subspace changes can be detected and the subspaces can be tracked with near-optimal delay, and (ii) the time complexity of doing this is the same as that of simple (non-robust) PCA. Our main result assumes piecewise constant subspaces (needed for identifiability), but we also provide a corollary for the case when there is a little change at each time. A second contribution is a novel non-asymptotic guarantee for PCA in linearly data-dependent noise. An important setting where this is useful is for linearly data dependent noise that is sparse with support that changes enough over time. The analysis of the subspace update step of our proposed robust ST solution uses this result.

==> Tex_Commands.tex <==


\setlength{\arraycolsep}{0.03cm}

%\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\seq}[1]{\left<#1\right>}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\essnorm}[1]{\norm{#1}_{\ess}}

%% THEOREM ENVIRON ---------------------------------------------------
%
%%\newtheorem{theorem}{Theorem}
%%\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{sigmodel}[theorem]{Asssumption}%{Model}%
%%\newtheorem{corollary}[theorem]{Corollary}
%%\newtheorem{definition}[theorem]{Definition}
%%\newtheorem{remark}[theorem]{Remark}
%%\newtheorem{example}[theorem]{Example}
%%\newtheorem{ass}[theorem]{Assumption}
%%\newtheorem{proposition}[theorem]{Proposition}


% THEOREM ENVIRON ---------------------------------------------------

%\newtheorem{theorem}{Theorem}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
%\newtheorem{fact}[theorem]{Fact}
\newtheorem{sigmodel}[theorem]{Asssumption}%{Model}%
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{ass}[theorem]{Assumption}
%\newtheorem{proposition}[theorem]{Proposition}

%from zcom.tex %\input{zcom}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\be}{\protect\[}
\newcommand{\ee}{\protect\]}
\newcommand{\bean}{\begin{eqnarray*} }
\newcommand{\eean}{\end{eqnarray*} }
\newcommand{\bea}{\begin{eqnarray} }
\newcommand{\eea}{\end{eqnarray} }
\newcommand{\ba}{\begin{align*} }
\newcommand{\ea}{\end{align*} }

\newcommand{\nn}{\nonumber}
%\newcommand{\ba}{\begin{array} }
%\newcommand{\ea}{\end{array} }
\newcommand{\re}{\mathbb{R}}
\newcommand{\n}{{\cal N}}
\newcommand{\nois}{g}
\newcommand{\epsbnd}{d(\alpha)}
\newcommand{\epsden}{d_{\mathrm{denom}}(\alpha)}




%commands from Dynamic CS and Modified-CS works
\newcommand{\rest}{\mathrm{rest}}
%{{T_\mathrm{rest}}}
\newcommand{\zetahat}{\hat{\zeta}}
%\newcommand{\sm}{\mathrm{small}}
\newcommand{\tDelta}{{\tilde{\Delta}}}
\newcommand{\tDeltae}{{\tilde{\Delta}_e}}
\newcommand{\tT}{{\tilde{T}}}
%\newcommand{\add}{{\cal A}}
%\newcommand{\rem}{{\cal R}}
%\newtheorem{sigmodel}{Signal Model}

\newcommand{\thr}{{\mathrm{thr}}}
\newcommand{\delthr}{{\mathrm{del-thr}}}
\newcommand{\delbound}{{b}}
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\Q}{{\cal Q}}

\newcommand{\CSres}{{\mathrm{CSres}}}
\newcommand{\diff}{{\mathrm{diff}}}
\newcommand{\Aset}{{\cal A}}
\newcommand{\Rset}{{\cal R}}
\newcommand{\Iset}{{\cal I}}
\newcommand{\Dset}{{\cal D}}
\newcommand{\Sset}{{\cal S}}
\newcommand{\Lset}{{\cal L}}
\newcommand{\Nset}{N}  %{{\cal N}}
\newcommand{\Nhat}{\hat{{\cal N}}}
\newcommand{\N}{{{\cal T}}}
%\newcommand{\del}{\text{del}}
%\newcommand{\Span}{\text{range}}
%\newcommand{\Phat}{\hat{P}}
%\newcommand{\that}{\hat{t}}
%\newcommand{\new}{{\text{new}}}
%\newcommand{\old}{{\text{old}}}
\newcommand{\dif}{{\text{dif}}}
%\newcommand{\thresh}{{\text{thresh}}}
%\newcommand{\Shat}{\hat{S}}
%\newcommand{\lhat}{\hat{\ell}}
\newcommand{\xhat}{\bm{\hat{x}}}
%\newcommand{\That}{\hat{\mathcal{T}}}
%\newcommand{\T}{\mathcal{T}}
%\newcommand{\SE}{\text{SE}}
\newcommand{\mat}{\mathrm{mat}}
%\newcommand{\train}{{\text{train}}}  %(recursive projected CS)
%\newcommand{\train}{{\text{0}}}  %(recursive projected CS)


\newcommand{\bl}{\begin{frame}}
\newcommand{\el} {\end{frame}}
\newcommand{\hd}{\frametitle}
%\newcommand{\sd}{\frametitle}
\newcommand{\cred}{\color{red}} % \bf
\newcommand{\cb}{\color{blue}}
\newcommand{\cbl}{\color{black}}
\newcommand{\cg}{\color{DarkGreen}}
\newcommand{\im}{\vspace{1mm} \item}
\newcommand{\vs}{\vspace{2mm}}
\newcommand{\vsl}{\vspace{1mm}}
\newcommand{\vsm}{\vspace{-2mm}}
\newcommand{\svdeq}{\overset{\mathrm{SVD}}=}
\newcommand{\evdeq}{\overset{\mathrm{EVD}}=}
\newcommand{\qreq}{\overset{\mathrm{QR}}=}


\newcommand{\supp}{\text{support}}
\newcommand{\tw}{\tilde{w}}


\renewcommand\thetheorem{\arabic{section}.\arabic{theorem}}

\newcommand{\tmax}{d} %t_{\mathrm{final}}}

%%% ReProCS Commands %%%%%%%%%%
\newcommand{\bbeta}{\beta}%{\tilde\beta}

\newcommand{\wt}{\bm{w}_t}
\newcommand{\mt}{\bm{m}_t}
\newcommand{\xt}{\bm{x}_t}
\newcommand{\x}{\bm{x}}
\newcommand{\xhatt}{\hat{\bm{x}}_t}
\renewcommand{\l}{\bm{\ell}}
\newcommand{\s}{\bm{s}}
\newcommand{\lt}{\bm{\ell}_t}
%\newcommand{\lhat}{\bm{\hat{\ell}}}
\newcommand{\lhat}{\hat{\bm{\ell}}}

\newcommand{\lhatt}{\hat{\l}_t}   %{\bm{y}_t} %{\y_t}
\newcommand{\yt}{\bm{y}_t}
\newcommand{\y}{\bm{y}}
\newcommand{\tty}{\tilde{\bm{y}}}
%\newcommand{\wt}{\bm{w}_t}
\newcommand{\w}{\bm{w}}
\renewcommand{\v}{{\bm{v}}}
\newcommand{\vt}{\bm{v}_t}

\renewcommand{\a}{\bm{a}}
\newcommand{\e}{\bm{e}} %{\bm{w}}  %
\newcommand{\bnu}{{\bm{\nu}}}
\newcommand{\et}{\bm{e}_t}%{\bm{w}_t}%
\newcommand{\Pt}{\bm{P}_t}
\newcommand{\Pj}{\bm{P}_{(j)}}
\newcommand{\Pjm}{\bm{P}_{(j-1)}}
\newcommand{\Pjs}{\bm{P}_{(j),*}}

\newcommand{\ttrain}{t_{\mathrm{train}}}
\newcommand{\rmnew}{\mathrm{new}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\ex}{\mathrm{ex}}

\newcommand{\Pjnew}{\bm{P}_{(j),\mathrm{new}}}
\newcommand{\at}{\bm{a}_t}
\newcommand{\ats}{\bm{a}_{t,*}}
\newcommand{\atnew}{\bm{a}_{t,\mathrm{new}}}
\newcommand{\I}{\bm{I}}
\newcommand{\Lamt}{\bm{\Lambda}_t}
\newcommand{\Lam}{\bm{\Lambda}}
\newcommand{\Lamtnew}{\bm{\Lambda}_{t,\mathrm{new}}}
\newcommand{\Lamtaunew}{\bm{\Lambda}_{\tau,\mathrm{new}}}
\newcommand{\Lamtstar}{\bm{\Lambda}_{t,*}}
\newcommand{\Lamtex}{\bm{\Lambda}_{t}}
%\newcommand{\bm\Sigma}{\bm{\Lambda}_{(j)}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\J}{\mathcal{J}}


\newcommand{\D}{\bm{D}}
\newcommand{\A}{\bm{A}}
\newcommand{\cM}{\hat{\bm{D}}}  % {\mathcal{\bm{M}}}
\newcommand{\cA}{\bm{D}}    %{\mathcal{\bm{A}}}
\newcommand{\cH}{\bm{H}}


\newcommand{\cs}{\text{cs}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\newset}{\mathrm{new-set}}
\newcommand{\old}{\mathrm{old}}
\newcommand{\Shat}{\hat{\bm{s}}}
\newcommand{\shat}{\hat{\bm{s}}}
\newcommand{\Lhat}{\hat{\bm{L}}}
%\newcommand{\lhat}{\l}

\newcommand{\Ltilde}{\ttilde{\bm{\ell}}}
\newcommand{\Ltil}{\ttilde{\bm{\ell}}}
\renewcommand{\P}{\bm{P}}
\newcommand{\U}{\bm{U}}
\newcommand{\V}{\bm{V}}
\newcommand{\R}{\bm{R}}
\newcommand{\ch}{{\mathrm{ch}}}
\newcommand{\fx}{{\mathrm{fix}}}
\newcommand{\rot}{{\mathrm{add}}} %{{\mathrm{rot}}}

\newcommand{\mG}{{\mathcal{G}}}
\newcommand{\G}{{\bm{G}}}
\newcommand{\Ghat}{\hat{\bm{G}}}


\renewcommand{\b}{\bm{b}}
\newcommand{\Phat}{\hat{\bm{P}}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Span}{\operatorname{span}} %{\operatorname{range}}
\newcommand{\del}{\mathrm{del}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\add}{\mathrm{add}}%{\mathrm{add}}
\newcommand{\basis}{\operatorname{basis}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\calc}{\mathcal{C}}
\newcommand{\full}{\mathrm{full}}
\newcommand{\cov}{\operatorname{Cov}}

\newcommand{\train}{\mathrm{train}}
\newcommand{\thresh}{\lambda_{\mathrm{thresh}}}  %{\mathrm{thresh}}  %{\hat{\lambda}^-}
\newcommand{\bbbetathresh}{\eta} %{\text{add-thresh}}
\newcommand{\That}{\hat{\mathcal{T}}}
\newcommand{\zetasp}{{\zeta_{*}^+}}
%\newcommand{\SE}{\mathrm{SE}}
\newcommand{\SE}{\sin\theta_{\max}}
\newcommand{\egam}{\Gamma^e}
\newcommand{\Ijk}{\mathcal{I}_{k}}
\newcommand{\that}{{\hat{t}}}
\newcommand{\rmend}{\mathrm{end}}
\newcommand{\M}{\bm{M}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\llceil}{\left\lceil}
\newcommand{\rrceil}{\right\rceil}
\newcommand{\llfloor}{\left\lfloor}
\newcommand{\rrfloor}{\right\rfloor}
\newcommand{\uhat}{{\hat{u}}}
%\newcommand{\lammin}{{\hat{\lambda}_{\train}^-}}
\newcommand{\lammin}{{\lambda}^-}
\newcommand{\lamtrain}{{\lambda}^-} %{{\hat{\lambda}_{\train}^-}}
\newcommand{\jhat}{j}%{\hat{\jmath}}

\newcommand{\rrho}{\rho}
%\newcommand{\Ijk}{\mathcal{I}_{k}}
\newcommand{\Ijkt}{\ttilde{\mathcal{I}}_{k}}
\newcommand{\ghatp}{\hat{g}}%{\hat{g}^+}
\newcommand{\calGjk}{\mathcal{G}_{k}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\Lamcl}{\bm{\Lambda}_{(j),\mathrm{cl}}}
\newcommand{\bnut}{{\bnu}_t}
\newcommand{\bmG}{\bm{G}}
%\newcommand{\L}{\bm{L}}
%\newcommand{\S}{\bm{S}}
\newcommand{\X}{\bm{X}}
\newcommand{\Y}{\bm{Y}}
\newcommand{\W}{\bm{W}}
\newcommand{\Z}{\bm{Z}}
\newcommand{\bE}{\bm{E}}
\newcommand{\F}{\bm{F}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bR}{\bm{R}}

\renewcommand{\H}{\bm{H}}


\newcommand{\outfrac}{\small{\text{max-outlier-frac}}}
\newcommand{\outfracrow}{\small{\text{max-outlier-frac-row}}}
\newcommand{\outfraccol}{\small{\text{max-outlier-frac-col}}}


\newcommand\diagmat[2]{\begin{bmatrix} #1 & \bm{0} \\ \bm{0} & #2\end{bmatrix}} %Usage: $\diagmat{a}{b}$
\newcommand{\one}{\bm{1}}
\newcommand{\polylog}{\mathrm{polylog}}

\newcommand{\matr}[2]{ \left[\begin{array}{cc}
     #1 \\
     #2
   \end{array}
  \right]
  }

\newcommand{\ed}{\mathrm{end}}
\newcommand{\termoneone}{{\mathrm{term11}}}
\newcommand{\SVD}{{SVD}}
\newcommand{\B}{\bm{B}}
\newcommand{\bdel}{b_0}%{b_{0,\del}}
\newcommand{\alphadel}{\alpha}%{\alpha_\del}
\renewcommand{\Re}{\mathbb{R}}

\newcommand{\iidsim}{\overset{\mathrm{iid}}{\sim}} 

==> norst_it_extensions.tex <==
\section{Extensions}\label{sec:extensions}
{\cred
mention that this has been published in TSP etc}

%In this section we provide three extensions that follow from our main result for RST. %We prove all the results in Appendix \ref{sec:proof_reprocs-pca-mc}.
%\subsubsection{Subspace change model with $r_\ch$ directions changing}
%If the subspace does indeed change in such a way that  only $r_\ch \le r$ directions change, we have the following corollary (that does not require knowing $r_\ch$).
%\begin{corollary}
% Suppose that $r_\ch \le r$ directions change at each $t_j$. Let $\dif:=\max_j \SE( \P_{j-1},\P_j)$.
%\bi
%%\item Let $\P_{j-1} \R_j = [ \P_{j-1,\fx}, \P_{j-1,\ch}]$ where $\R_j$ is a rotation matrix. This means that $\P_j = [\P_{j-1,\fx}, \P_{j-1,\chd}]$ and so $\SE(\P_{j-1},\P_j) = \SE( \P_{j-1,\ch}, \P_{j,\chd})$. Let $\dif:=\max_j \SE( \P_{j-1,\ch}, \P_{j,\chd})$.
%\item Modify NORST as follows: let $\Phat_{(t)}$  be to a basis matrix for $\Span([\Phat_{j-1}, \Phat_{j,k}])$.
%\item Then, Theorem \ref{thm1} holds with the subspace change condition replaced by the following relaxed lower bound: $\xmint \ge C (\zz \sqrt{r \lambda^+} +  \semax\sqrt{r_\ch \lambda_\ch^+})$.
%\ei
%\end{corollary}
%In the above, $\lambda_\ch^+$ is the maximum eigenvalue along the changing directions\footnote{Proof: The only change is in the first step of the projected-CS proof. With $\Phat_{(t)}$ set as above, in the $k$-th subspace update interval, $\|\bm\Psi \lt\| \le 2\zz \sqrt{r \lambda^+} + 0.3^{k-1} (\zz + \semax) \sqrt{r_\ch \lambda_\ch^+}$.}  (this is often much smaller than $\lambda^+$). When $r_\ch=1$, the above corollary recovers the guarantee of s-ReProCS given in \cite{rrpcp_dynrpca}.
%
\subsection{Static Robust PCA}
A useful corollary of our result for RST is that NORST is also the {first online algorithm that provides a provable finite sample guarantee for the static Robust PCA problem}. %A short version of this result appeared in \cite{rrpcp_merop}.
Static RPCA is our problem setting with $J=1$, or in other words, with $\lt = \P \at$.
%% and $t_2 = \infty$. That is, we observe $n$-dimensional data vectors,
%\begin{align}\label{eq:strpca}
%\yt = \lt + \xt + \wt,\ t = 1,\ 2,\ \cdots,\ \tmax
%\end{align}
%where $\lt = \P \at$, $\xt$'s are sparse and $\wt$ is small, unstructured noise. The assumptions on $\xt$ and $\wt$ are the same as in the RST/Dynamic RPCA problem. Although this problem has been extensively studied, it has received considerably less treatment in the online setting.
A recent work, \cite{xu_nips2013_1}, developed an online stochastic optimization based reformulation of PCP, called ORPCA, to solve this. Their paper provides only a partial guarantee because the guarantee assumes that the intermediate algorithm estimates, $\Phat_{(t)}$, are full-rank. Moreover the guarantee is only asymptotic.  Instead our result given below is a complete guarantee and is non-asymptotic.
%convergence guarantees and do not derive precise error bounds as function of number of samples.

%\subsubsection{Static RPCA} We have the following guarantee.
%The static (original) RPCA problem, is our model with $J=1$ (no subspace change) and thus with $\rmat=r$. Thus, NORST (without the subspace change detection step) also provides a new provably online (after initialization), fast, nearly memory-optimal, solution to static RPCA that allows many more outliers per row in some rows.
\begin{corollary}[Static RPCA]\label{thm:rpca}
Consider Algorithm \ref{norst_basic} with $t_2=\infty$. Theorem \ref{thm1} holds with following modification: replace the slow subspace change assumption with a fixed subspace $\P$. Everything else remains as is, but with $r \equiv \rmat$. Under the assumptions of Theorem \ref{thm1}, all the conclusions hold with same probability. The time and memory complexity  are $O(n d r \log(1/\epsilon))$ and $O(n r \log n \log(1/\epsilon))$.
\end{corollary}
%To the best of our knowledge, this is the first provable guarantee for static RPCA. %that holds under ``weakened'' RPCA assumptions, fixed subspace, a main extra assumption of a lower bound on most outlier magnitudes and mutual independence, element-wise bounded-ness, identical and diagonal covariance assumption on $\at$'s. To bring out a semantic difference, we use {\em static RPCA} to refer to the problem where the ``true subspace'' in which the data lies is fixed. This is not required by {\em original RPCA} methods which can, in principle, tolerate a few sudden subspace changes. We have the following result for the static RPCA problem.

In applications such as ``robust'' dimensionality reduction \cite{dimreduce_app1, dimreduce_app2} where the objective is to just obtain the top-$r$ directions along which the variability of data is maximized, we only need the first $K\alpha = Cf^2r\log n \log(1/\zz)$ samples to obtain an $\zz$-accurate subspace estimate. If only these are used, the time complexity reduces to $O(n K \alpha r \log(1/\zz)) = O(n r^2 \log n \log^2(1/\epsilon))$. This is faster than even NO-RMC \cite{rmc_gd} and does not require $\tmax \approx n$; of course it requires the other extra assumptions discussed earlier.
%This ``undersampling'' allows us to provide {\em the second linear-time algorithm for PCA in the presence of gross outliers}. In fact from Corollary \ref{cor:rpca}, we notice that the time complexity is $O(n r^2 \log n \log^2(1/\zz))$ which improves upon the fastest known result due to \cite{rmc_gd} by a factor of $O(r \log n)$.

%\begin{corollary}[Static Outlier-Robust-PCA]\label{cor:rpca}
%If the goal is only computing the Principal Components for the fixed subspace problem, Algorithm \ref{norst_basic}, applied to the first $O(K\alpha) = O(r f^2 \log n \log(1/\epsilon))$ samples returns an $\epsilon$-accurate subspace estimate. In this case, the time complexity reduces to $O(n r^2 \log n \log^2(1/\epsilon))$.
%\end{corollary}

\subsection{Subspace Tracking with Missing Data (ST-missing) and Dynamic Matrix Completion}
Another useful corollary of our result is a guarantee for the ST-missing problem.
%This problem has been studied in \cite{petrels, grouse}, however, as mentioned earlier, these are partial guarantees, and impose several assumptions on intermediate algorithm parameters. ST-missing is closely related to the matrix completion (MC) problem that has also been extensively studied in the literature \cite{matcomp_first, lowrank_altmin} and in fact the version studied in \cite{petrels, grouse} is exactly the same as the MC problem since it assumes a single unknown subspace.
%Although, there is a vast body of provable literature which analyse MC, most of these assume that the set of observed entries is generated uniformly at random.  Some recent works that do not require a uniform random model, include \cite{coherent_mc} which uses leverage score based sampling, \cite{powerlaw_mc} which requires that the set of observed entries follows power-law distributed graphs, and finally, \cite{universal_mc} assumes that set of observed entries are generated from the edges of a bipartite graph with a large spectral gap. To the best of our knowledge, Corollary \ref{cor:stmiss} is the first provable guarantee for the ST-missing problem.
%
Consider the subspace tracking with missing data (ST-missing) problem. By setting the missing entries at time $t$ to zero, and by defining $\T_t$ to be the set of missing entries at time $t$, we observe $n$-dimensional vectors that satisfy
\bea
\yt := \lt - \itt \itt{}' \lt, \text{ for } t = 1, 2, \dots, \tmax.
\label{eq:dynmc}
\eea
with $\xt \equiv \itt \itt{}' \lt$. This can be interpreted as a special case of the RST problem where the set $\T_t$ is known. Because there are no sparse corruptions (outliers), there is no $\xmint$. Thus the initialization error need not be $O(1/\sqrt{r})$ (needed in the RST result to ensure a reasonable lower bound on $\xmint$) and so one can even use random initialization. We assume that the initialization is obtained using the Random Orthogonal Model described in \cite{matcomp_candes}. As explained in \cite{matcomp_candes}, a basis matrix generated from this model is already $\mu$-incoherent. We have the following corollary. The only change in its proof is the proof of the first subspace update interval for the $j=0$ case.
%We prove it in Appendix.

%Thus the NORST algorithm applies with the $l_1$-min and support estimation steps removed and replaced by $\That_t=\T_t$ (which is now given). Since $\T_t$ is now given, we do not need an $\xmint$ lower bound. This, in turn, implies that we do not need a ``good" initial estimate of $\P_0$. This was needed in case of RST to ensure that the lower bound on $\xmint$ imposed by the initialization assumption was reasonable. Thus, we can use a random initialization of $\Phat_0$ as long as it satisfies incoherence. One way to ensure this is to  generate it from a random orthogonal model \cite{matcomp_candes}. This means the following: $\Phat_\init$ is the orthonormalized version of an $n \times r$ matrix with each column generated i.i.d. from the unit hypersphere in $\Re^n$.

%Second, replace the initialization via AltProj by  using the left singular vectors of a matrix drawn from the Random Orthogonal Model (ROM) \cite{matcomp_candes}, since it is shown that matrices from these ensembles satisfy incoherence with high probability. The most simple ROM is where the entries of the matrix are drawn independently from a Gaussian distribution with appropriately normalized variance??.

\begin{corollary}[ST-missing]\label{cor:stmiss}
Consider NORST-Random (Algorithm \ref{algo:auto-dyn-mc}). If the assumptions of Theorem \ref{thm1} on $\at$ and $\vt$ hold, $\P_j$'s are $\mu$-incoherent,  $t_{j+1}-t_j > (K+2)\alpha$, $\Delta < 0.8$, the outlier fraction bounds given in Theorem \ref{thm1} hold, and if, for $t \in [t_0,t_1]$, $\outfraccol \le c/ (\log n)$, then all conclusions of Theorem \ref{thm1} on $\Phat_{(t)}$ and on $\lt$ hold with the same probability.
\end{corollary}
To our knowledge, the above is the first complete non-asymptotic guarantee for ST-missing; and the first result that allows changing subspaces. All existing guarantees are either partial guarantees (make assumptions on intermediate algorithm estimates), e.g., \cite{local_conv_grouse}, or provide only asymptotic results \cite{past,petrels}.
Moreover, from a dynamic matrix completion viewpoint, it is also giving a matrix completion solution without assuming that the set of observed entries is generated from a uniform or a Bernoulli model. Of course the tradeoff is that it needs many more observed entries. All these points will be discussed in detail in follow-up work where we will also numerically evaluate NORST-random for this problem.

%In our result presented in Corollary \ref{cor:stmiss}, we (i) provide guarantees for the changing subspace model, (ii) only impose an upper bound on the fraction of missing entries rather than assuming a model on how the outlier support set is generated. However, the tradeoff is that we require many more samples than best known guarantees. We now formally define the problem, and present the Algorithm and main result.


\begin{algorithm}[t!]
\caption{NORST-Random for subspace tracking with missing data (ST-missing)}
%Let $\hat{\L}_{t; \alpha} := [\lhat_{t-\alpha + 1}, \cdots, \lhatt]$. $\SVD_r[\M]$ computes the top of $r$ left singular vectors of the matrix $\M$.
%}
% This is the actual version of the algorithm we implement and analyse. Let $\L_{t;\alpha} := [\lhat_{t-\alpha + 1}, \cdots, \lhatt]$.}
\label{algo:auto-dyn-mc}
%\begin{algorithmic}[1]
%\algrenewcommand\algorithmicindent{1em}
%\STATE \textbf{Input}:  $\yt$,  \textbf{Output}:  $\shatt$, $\lhatt$,  $\Phat_{(t)}$
%\STATE \textbf{Parameters:} $\omega_{supp}$, $K$, $\alpha$, $\xi$, $r$, $\lthres$
Algorithm \ref{norst} with the following changes
\ben
\item Replace line 3 with: compute $\Phat_0 \leftarrow \Phat_\init \leftarrow \text{Generate an $n \times r$ basis matrix from the random orthogonal model}$;  $\tildej~\leftarrow~1$, $k~\leftarrow~1$

\item Replace line 6 with the following
\bi
\item $\bpsi \leftarrow \bm{I} - \hat{\pt}_{(t-1)}\hat{\pt}_{(t-1)}{}'$; $\tty_t \leftarrow \bpsi \yt$;
 $\xhat_t \leftarrow \I_{\T_t} ( \bpsi_{\T_t}{}' \bpsi_{\T_t} )^{-1} \bpsi_{\T_t}{}'\tty_t$;  $\hat{\bm{\ell}}_t \leftarrow \yt - \hat{\bm{x}}_t$.
\ei
\een
%\end{algorithmic}
\end{algorithm}


%Since $\xt$ is not even present in this case, we do not need the $\xmint$ lower bound. For this reason, we can allow random initialization (which does not guarantee $\SE(\Phat_\init,\P_0)$ to be $O(1/\sqrt{r})$. Recall that this was (implicitly) needed in the RST result to make the $\xmint$ lower bound reasonable.

%Additionally, as in the case of static RPCA, if we assume $J=1$ and $t_2 = \infty$, the ST-missing problem translates into a Matrix Completion problem with fixed subspace. Our guarantee, is the first result that provides a complete guarantee for MC without any assumption on set of observed entries.

\subsection{Fewer than $r$ directions change}
It is possible to relax the lower bound on outlier magnitudes if not all of the subspace directions change at a given subspace change time. Suppose that only $r_\ch < r$ directions change. When $r_\ch=1$, we recover the guarantee of \cite{rrpcp_dynrpca} but for NORST (which is a simpler algorithm than s-reprocs).
%we impose a slightly more stringent model on how the subspace changes. Furthermore, this result is the model considered in s-ReProCS \cite{rrpcp_dynrpca} and as we show below, our result recovers their result. Concretely, if the subspace changes such that only $r_\ch \ll r$ directions change at each subspace change time, i.e., under the same notation of Theorem \ref{thm1} the subspace changes as follows, or all $j$,

Let $\P_{j-1, \fx}$ denote a basis for the fixed component of $\P_{j-1}$ and let $\P_{j-1,\ch}$ denote a basis for its changing component. Thus,
$\P_{j-1} \R = [ \P_{j-1,\fx}, \P_{j-1,\ch}]$, where $\bm{R}$ is a $r \times r$ rotation matrix. %$\P_{j-1, \fx}$ is the ``fixed component'' with dimensions $n \times (r - r_\ch)$, $\P_{j-1, \ch}$ is the ``changing component'' with dimensions $n \times r_\ch$. and $\bm{R}$ is a $r \times r$ rotation matrix. Further
We have
\begin{align}\label{eq:rchdef1}
\P_j = [\P_{j-1,\fx}, \P_{j,\chd}]
\end{align}
where $\P_{j, \chd}$ is the changed component and has the same dimension as $\P_{j-1, \ch}$. Thus,
\begin{align}\label{eq:rchdef2}
\SE(\P_{j-1},\P_j) = \SE( \P_{j-1,\ch}, \P_{j,\chd})
\end{align}
and so $\Delta = \max_j \SE(\P_{j-1},\P_j) = \max_j \SE( \P_{j-1,\ch}, \P_{j,\chd})$.
Let $\lambda_{\ch}^+$ denote the largest eigenvalue along any direction in $\P_{j,\chd}$.
\begin{corollary}\label{cor:rch}
In Algorithm \ref{algo:auto-reprocs-pca}, replace line 17 by $\Phat_{(t)} \leftarrow \basis(\Phat_{j-1}, \Phat_{j, k})$. For basis matrices $\P_1, \P_2$, we use $\P = \basis(\P_1, \P_2)$ to mean that $\P$ is a basis matrix with column span equal to the column span of $[\P_1, \P_2]$.
Assume that  \eqref{eq:rchdef1} and \eqref{eq:rchdef2} hold. Also assume that the conditions of Theorem \ref{thm1} holds with the lower bound on $\xmint$ relaxed to $\xmint \ge C (\zz \sqrt{\eta (r - r_\ch) \lambda^+} + (\zz + \Delta) \sqrt{\eta r_\ch \lambda_\ch^+})$.
Then, all conclusions of Theorem \ref{thm1} hold.% with the same probability.
\end{corollary}
%A further relaxation on the lower bound as demonstrated in Remark \ref{rem:r_change} is trivially possible even in this special case.


==> norst_supp_sims.tex <==
\section{Synthetic Experiments Extra Details}
All time comparisons are performed on a Desktop Computer with Intel$^{\textsuperscript{\textregistered}}$ Xeon E$3$-$1240$ $8$-core CPU @ $3.50$GHz and $32$GB RAM and all synthetic data experiments are averaged over $100$ independent trials. The codes are available at \url{https://github.com/praneethmurthy/NORST}. 
\subsubsection{Algorithm Parameters}
For $l_1$ minimization we used the \texttt{YALL-1} toolbox and set the tolerance to $10^{-4}$. For the least-squares step we use the Conjugate Gradient Least Squares instead of the well-known ``backslash'' operator in \texttt{MATLAB} since this is a well conditioned problem. For this we set the tolerance as $10^{-10}$ and the number of iterations as $10$. We have not done any code optimization such as use of \texttt{MEX} files for various sub-routines to speed up our algorithm. % \cite{yall1}


\subsubsection{Data Generation}
For the phase transition plot, for each pair of $\{b_0, r\}$ we used the Bernoulli model for sparse support generation, the low rank matrix is generated exactly as done in the previous experiments with the exception that again to provide an equal footing, we increased the ``subspace change'' by setting $\gamma_1$ and $\gamma_2$ to $10$ times the value that was used in the previous experiment. For the first $t_\train$ frames we used $b_0 = 0.02$. We provide the phase transition plots for both algorithm in Fig. \ref{fig:Comparison}. Here, white represents success while black represents failure. As can be seen, NORST is able to tolerate a much larger fraction of outlier-per-row as compared to AltProj.


\subsubsection{Real Data descriptions}
{\em Meeting Room (MR) dataset}: The meeting room sequence is set of $1964$ images of resolution $64 \times 80$. The first $1755$ frames consists of outlier-free data. Henceforth, we consider only the last $1209$ frames. For NORST, we used $t_\train=400$. In the first $400$ frames, a person wearing a black shirt walks in, writes something on the board and goes back. In the subsequent frames, the person walks in with a white shirt. This is a challenging video sequence because the color of the person and the color of the curtain are hard to distinguish. NORST is able to perform the separation at around $43$ frames per second. We present the results in Fig. \ref{fig:mr_full}

{\em Lobby (LB) dataset}: This dataset contains $1555$ images of resolution $128 \times 160$. The first $341$ frames are outlier free. Here we use the first $400$ ``noisy'' frames as training data. The Alt Proj algorithm is used to obtain an initial estimate with rank, $r = 40$. The parameters used in all algorithms are exactly the same as above. NORST achieves a ``test'' processing rate of $16$ frames-per-second. 

%--------------------------------------------


